DFW-PP: Dynamic Feature Weighting based Popularity Prediction for Social Media Content

The increasing popularity of social media platforms makes it important to study user engagement, which is a crucial aspect of any marketing strategy or business model. The over-saturation of content on social media platforms has persuaded us to identify the important factors that affect content popularity. This comes from the fact that only an iota of the humongous content available online receives the attention of the target audience. Comprehensive research has been done in the area of popularity prediction using several Machine Learning techniques. However, we observe that there is still significant scope for improvement in analyzing the social importance of media content. We propose the DFW-PP framework, to learn the importance of different features that vary over time. Further, the proposed method controls the skewness of the distribution of the features by applying a log-log normalization. The proposed method is experimented with a benchmark dataset, to show promising results. The code will be made publicly available at https://github.com/chaitnayabasava/DFW-PP.

==> supplementary_material.tex <==
% \documentclass[sigconf]{acmart}

% \usepackage[english]{babel}

% \usepackage{graphicx}
% \usepackage{booktabs} % For formal tables
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{lipsum}
% Copyright
%\setcopyright{none}
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
% \setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}


% DOI
% \acmDOI{10.475/978_1}

% ISBN
% \acmISBN{978-1-4503-6615-1}
%\acmISBN{123-4567-24-567/08/06}

%Conference
% \acmConference[ICVGIP'18]{11th Indian Conference on Computer Vision, Graphics and Image Processing}{Dec. 2018}{Hyderabad, India}
% \acmYear{2018}
% \copyrightyear{2018}


% \acmArticle{4}
% \acmPrice{15.00}

% These commands are optional
%\acmBooktitle{Transactions of the ACM Woodstock conference}
% \editor{Anoop M. Namboodiri}
% \editor{Vineeth Balasubramanian}
% \editor{Amit Roy-Chowdhury}
% \editor{Guido Gerig}


% \begin{document}

% \begin{titlepage}
% \begin{center}
%     \Huge \textbf{Supplementary Material for\\DFW-PP: Dynamic Feature Weighting based Popularity Prediction for Social Media Content}
        
%     \vspace{0.4cm}
%     \normalsize
%     \textbf{Paper ID: 181}
    
%     \vfill
    
% \end{center}
% \end{titlepage}

% \onecolumn
% If the list of authors is too long for headers, add the following line:
% \renewcommand{\shortauthors}{Paper ID: 181}
% \maketitle

\section{Appendix}


\begin{figure*}
\begin{center}
  \includegraphics[width=\linewidth]{ICVGIP18-CameraReady/images/m2_50.jpg}
\end{center}
\caption{K-means clustering elbow method graphs for K's range [1, 50]}
\label{fig:elbow_50}
\end{figure*}

\begin{figure*}
\begin{center}
  \includegraphics[width=\linewidth]{ICVGIP18-CameraReady/images/m1_10.jpg}
\end{center}
\caption{K-means clustering elbow method graphs for K's range [1, 10]}
\label{fig:elbow_10}
\end{figure*}

\begin{table*}
\centering
\caption{The performance of the proposed framework in terms of the Case A \& B as compared to the existing normalization techniques ($s_{scale}$ normalization). Random Forest is used for all the evaluation settings.}
\label{table:normalizationresultsAB}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Scaling}\\\textbf{Method}\end{tabular}} & \multicolumn{4}{c|}{\textbf{Case A}} & \multicolumn{4}{c|}{\textbf{Case B}} \\ 
\cline{2-9}
 & $tRMSE_{mean}$ & $tRMSE_{median}$ & $tMAE_{mean}$ & $tMAE_{median}$ & $tRMSE_{mean}$ & $tRMSE_{median}$ & $tMAE_{mean}$ & $tMAE_{median}$ \\ 
\hline
No scaling & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.152±0.03 &   1.626±0.023  & 1.941±0.025 & 1.447±0.019 \\ 
\hline
log & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.138±0.034 & 1.619±0.036 & 1.924±0.035 & 1.432±0.036 \\ 
\hline
\begin{tabular}[c]{@{}c@{}}log(scale/30 \\+ 0.1)\end{tabular} & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.145±0.039 & 1.62±0.035 & 1.934±0.035 & 1.436±0.031 \\ 
\hline
Ortis et al. & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.145±0.034 & 1.621±0.036 & 1.928±0.034 & 1.434±0.037 \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Proposed\\ normalization \end{tabular}& 1.608±0.014\textbf{} & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.146±0.023 & 1.624±0.029 & 1.934±0.018 & 1.442±0.02 \\
\hline
\end{tabular}
\end{table*}
% \usepackage{multirow}
\begin{table*}
\centering
\caption{The performance in terms of the Case A \& B metrics for different classification and regression modeling techniques}
\label{table:mainresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Case A}}                                & \multicolumn{4}{c|}{\textbf{Case B}}                                 \\ 
\cline{2-9}
                                & $tRMSE_{mean}$ & $tRMSE_{median}$ & $tMAE_{mean}$ & $tMAE_{median}$ & $tRMSE_{mean}$ & $tRMSE_{median}$ & $tMAE_{mean}$ & $tMAE_{median}$  \\ 
\hline
XGBoost                         & 1.608±0.014~   & ~1.221±0.024     & 1.401±0.014   & 1.053±0.02~     & ~2.217±0.027   & ~1.66±0.029      & ~2.003±0.024  & 1.479±0.023~     \\ 
\hline
LightGBM                        & 1.608±0.014~   & ~1.221±0.024     & 1.401±0.014   & 1.053±0.02~     & 2.196±0.038    & 1.64±0.032       & 1.983±0.035   & 1.462±0.03       \\ 
\hline
Bayesian                       & 1.608±0.014    & ~1.221±0.024~    & ~1.401±0.014  & 1.053±0.02      & 2.304±0.039~   & 1.722±0.037~     & 2.087±0.028   & ~1.535±0.028~    \\ 
\hline
SVM                            & ~1.608±0.014   & ~1.221±0.024~    & 1.401±0.014   & 1.053±0.02~     & ~2.272±0.041   & 1.684±0.032      & 2.059±0.033   & 1.504±0.023~     \\ 
\hline
Resnet 1D                         & 1.608 ± 0.025         & 1.221 ± 0.026            & 1.401 ± 0.023        & 1.053±0.02~            & 2.295 ± 0.047         & 1.703 ± 0.038            & 2.078 ± 0.047        & 1.518 ± 0.034             \\ 
\hline
% paper                          & \textbf{}      & \textbf{}        & \textbf{}     & \textbf{}       & \textbf{}      & \textbf{}        & \textbf{}     & \textbf{}        \\
% reproduced & 0.595±0.006 &  0.487±0.002 & 0.479±0.005 & 0.389±0.002 &  2.091±0.023  & 1.649±0.016  & 1.85±0.021 & 1.412±0.022   \\
% \hline
RF                             & 1.608±0.014~   & ~1.221±0.024~~   & 1.401±0.014   & 1.053±0.02      & 2.146±0.023~   & ~1.624±0.029     & 1.934±0.018   & 1.442±0.02~      \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!t]
\centering
\caption{The performance in terms of the Case A \& B metrics for different time period lengths}
\label{table:caseABtime}
  \begin{tabular}{c|cccc|cccc}%{SSSSSSSlSSSSSSSS} % {c|cccc|cccc}
    \toprule
    {\textbf{Period Length}} & \multicolumn{4}{|c|}{\textbf{Case A}} &
      \multicolumn{4}{c}{\textbf{Case B}} & 
      \cmidrule(lr){2-5}\cmidrule(lr){6-9}
      & \multicolumn{1}{|c}{$tRMSE_{mean}$} & {$tRMSE_{median}$} & {$tMAE_{mean}$} & \multicolumn{1}{c|}{$tMAE_{median}$} &  {$tRMSE_{mean}$} & {$tRMSE_{median}$} & {$tMAE_{mean}$} & {$tMAE_{median}$} \\
      \midrule
    
    \multicolumn{1}{c|}{5} & \multicolumn{1}{c}{1.451±0.023} & 1.089±0.019 & 1.343±0.023 & 
    \multicolumn{1}{c|}{0.998±0.015} & \multicolumn{1}{c}{1.978±0.046} & 1.482±0.033 & 1.876±0.048 & 1.39±0.032\\
    
    \multicolumn{1}{c|}{10} & \multicolumn{1}{c}{1.608±0.014} & 1.221±0.024 & 1.401±0.014 & 
    \multicolumn{1}{c|}{1.053±0.02} & \multicolumn{1}{c}{2.153±0.037} & 1.625±0.033 & 1.941±0.033 & 1.441±0.028\\
    
    \multicolumn{1}{c|}{15} & \multicolumn{1}{c}{1.713±0.011} & 1.293±0.09 & 1.439±0.01 & 
    \multicolumn{1}{c|}{1.079±0.007} & \multicolumn{1}{c}{2.284±0.005} & 1.731±0.003 & 1.983±0.005 & 1.491±0.0\\
    
    \multicolumn{1}{c|}{30} & \multicolumn{1}{c}{1.948±0.049} & 1.499±0.032 & 1.509±0.033 &
    \multicolumn{1}{c|}{1.138±0.021} & \multicolumn{1}{c}{2.689±0.073} & 2.044±0.031 & 2.083±0.05 & 1.573±0.028\\

    \bottomrule
  \end{tabular}
\end{table*}
% \begin{table*}
% \centering
% % \captionsetup{labelformat=empty}
% \caption{Comparison of Case A \& Case B - Time Period}
% \label{table:caseABtime}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{Period }\\\textbf{Length} \end{tabular}} & \multicolumn{4}{c|}{\textbf{Case A} } & \multicolumn{4}{c|}{\textbf{Case B} } \\ 
% \cline{2-9}
%  & $tRMSE_{mean}$ & $tRMSE_{median}$ & $tMAE_{mean}$ & $tMAE_{median}$ & $tRMSE_{mean}$ & $tRMSE_{median}$ & $tMAE_{mean}$ & $tMAE_{median}$ \\ 
% \hline
% 5 & 1.451±0.023 & 1.089±0.019 & 1.343±0.023 & 0.998±0.015 & 1.978±0.046 & 1.482±0.033 & 1.876±0.048 & 1.39±0.032 \\ 
% \hline
% 10 & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.153±0.037 & 1.625±0.033 & 1.941±0.033 & 1.441±0.028 \\ 
% \hline
% 15 & 1.713±0.011 & 1.293±0.09 & 1.439±0.01 & 1.079±0.007 & 2.284±0.005 & 1.731±0.003 & 1.983±0.005 & 1.491±0.0\\ 
% \hline
% 30 & 1.948±0.049 & 1.499±0.032 & 1.509±0.033 & 1.138±0.021 & 2.689±0.073 & 2.044±0.031 & 2.083±0.05 & 1.573±0.028 \\
% \hline
% \end{tabular}
% }
% \end{table*}

\begin{table*}
\centering
\caption{The performance of the proposed normalization technique($s_{scale}$ normalization) in terms of the Case A \& B metrics for different values of c. Random Forest is used for all the evaluation settings.}
\label{table:normalizationresultsforc2}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Scaling}\\\textbf{Method}\end{tabular}} & \multicolumn{4}{c|}{\textbf{Case A}}                                                                  & \multicolumn{4}{c|}{\textbf{Case B}}                                                                                                                                           \\ 
\cline{2-9}
                                                                                            & $tRMSE_{mean}$         & $tRMSE_{median}$     & $tMAE_{mean}$         & $tMAE_{median}$     & $tRMSE_{mean}$         & $tRMSE_{median}$     & $tMAE_{mean}$        & $tMAE_{median}$                                                                           \\ 
% \hline
% Ortis et al.                                                                                      & ~10.532±0.101~           & ~8.025±0.063~           & ~10.299±0.102~          & 7.851±0.049~           & 11.059±0.095             & ~8.522±0.043~           & ~10.823±0.095~          & ~8.364±0.045~                                                                                   \\ 
\hline

c = 0.5 &1.608±0.014   &  1.221±0.024  & 1.401±0.014  &  1.053±0.02 &  2.144±0.03  &  1.623±0.034  &1.933±0.024 & 1.44±0.025                                                       \\ 
\hline

c = 0.1                                                                                    & 1.608±0.014  & 1.221±0.024  & 1.401±0.014  & 1.053±0.02 &

 2.147±0.036  & 1.625±0.034 & 1.935±0.031 & 1.445±0.029                                                                                   \\ 
\hline
c = one & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.145±0.025 & 1.622±0.031 & 1.934±0.021 & 1.442±0.027 \\
\hline 
% \begin{tabular}[c]{@{}c@{}} c=prathyush  \end{tabular}                                 & \textbf{8.773~±~0.053} & \textbf{6.066±0.009} & \textbf{~8.564±0.056} & \textbf{5.927±0.015~~} & \textbf{~9.048±0.077~} & \textbf{6.362±0.036} & \textbf{8.831±0.082} & \textbf{6.205±0.041}   \\
% \hline

\begin{tabular}[c]{@{}c@{}}log(scale/30 \\+ 0.1)\end{tabular} &  1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.145±0.039 & 1.62±0.035 & 1.934±0.035 & 1.436±0.031 \\ 
\hline
\begin{tabular}[c]{@{}c@{}}log(scale/30\\+ 0.5)\end{tabular} & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.155±0.029 & 1.622±0.032 & 1.943±0.025 & 1.441±0.025 \\ 
\hline
 \begin{tabular}[c]{@{}c@{}}log(scale/30\\+ 1) \end{tabular} & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 & 1.053±0.02 & 2.145±0.034 & 1.621±0.036 & 1.928±0.034 & 1.434±0.037 \\ 
\hline

\end{tabular}
\end{table*}

% \begin{table*}
% \centering
% \caption{Comparison of Case A and Case B - Cluster Size}
% \label{table:mainresults}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
% \hline
% \multirow{2}{*}{ \textbf{Cluster Size} } & \multicolumn{4}{c|}{\textbf{Case A} } & \multicolumn{4}{c|}{\textbf{Case B}} \\ 
% \cline{2-9}
%  & $tRMSE_{mean}$  & $tRMSE_{median}$  & $tMAE_{mean}$  & $tMAE_{median}$  & $tRMSE_{mean}$  & $tRMSE_{median}$  & $tMAE_{mean}$  & $tMAE_{median}$  \\ 
% \hline
% 2 & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 &  1.053±0.02 & 2.146±0.023   &   1.624±0.029 & 1.934±0.018 &  1.442±0.02 \\
% \hline
% 3 & 1.31±0.013   &   0.994±0.015 & 1.12±0.013 & 0.835±0.011 &  2.066±0.021   &   1.572±0.005 & 1.849±0.018 & 1.389±0.002 \\
% \hline
% 5 & 1.058±0.01   &   0.816±0.001 & 0.883±0.008 & 0.677±0.003 & 2.037±0.018   &   1.572±0.005 & 1.811±0.014 & 1.377±0.008 \\
% \hline
% 25 & 0.68±0.004   &   0.551±0.006 & 0.551±0.003 & 0.447±0.004 & 2.075±0.013   &   1.638±0.009 & 1.833±0.01 & 1.404±0.009 \\
% \hline
% 30 & 0.657±0.018   &   0.531±0.009 & 0.53±0.015 & 0.425±0.008 & 2.089±0.042   &   1.635±0.013 & 1.849±0.04 & 1.412±0.017 \\
% \hline
% 45 & 0.595±0.006   &   0.487±0.002 &  0.479±0.005 & 0.389±0.002 & 2.105±0.018   &   1.655±0.012 & 1.863±0.015 & 1.423±0.015 \\
% \hline
% 50 & 0.58±0.008   &   0.474±0.004 & 0.465±0.006 & 0.375±0.003 & 2.097±0.016   &   1.657±0.012 & 1.852±0.016 &  1.417±0.01 \\
% \hline
% \end{tabular}
% \end{table*}

\begin{table*}
\centering
\caption{The performance in terms of the Case A \& B metrics for different combinations of cluster sizes}
\label{table:mainresults}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{ \textbf{Cluster Size} } & \multicolumn{4}{c|}{\textbf{Case A} } & \multicolumn{4}{c|}{\textbf{Case B} } \\ 
\cline{2-9}
 & $tRMSE_{mean}$  & $tRMSE_{median}$  & $tMAE_{mean}$  & $tMAE_{median}$  & $tRMSE_{mean}$  & $tRMSE_{median}$  & $tMAE_{mean}$  & $tMAE_{median}$  \\ 
\hline
(2, 2, 2) & 1.608±0.014 & 1.221±0.024 & 1.401±0.014 &  1.053±0.02 & 2.146±0.023   &   1.624±0.029 & 1.934±0.018 &  1.442±0.02 \\
\hline
(2, 2, 3) &	1.56±0.013 & 1.185±0.022 & 1.36±0.014 & 1.02±0.018 &	2.134±0.038 & 1.61±0.029 & 1.922±0.033 & 1.423±0.024 \\
\hline
(3, 3, 3) &	1.31±0.013 & 0.994±0.015 & 1.12±0.013 & 0.835±0.011	& 2.066±0.008 & 1.573±0.007 & 1.85±0.008 & 1.386±0.002 \\
\hline
% 5 & 8.653±0.106   &   5.981±0.043 & 8.452±0.112 & 5.845±0.051 & 8.983±0.102   &   6.299±0.051 & 8.758±0.103 & 6.132±0.048 \\
(3, 3, 4) &	1.281±0.017 & 0.973±0.018 & 1.096±0.016 & 0.818±0.014 &	2.066±0.017 & 1.572±0.007 & 1.846±0.017 & 1.384±0.004 \\
\hline

(3, 2, 4) & 1.39±0.017 & 1.06±0.019 & 1.198±0.017 & 0.9±0.014 & 2.047±0.011 & 1.562±0.008 & 1.828±0.009 & 1.37±0.003 \\

\hline
(3, 2, 3) &	1.419±0.013 & 1.08±0.016 & 1.222±0.013 & 0.917±0.01 & 2.045±0.012 & 1.555±0.01 & 1.829±0.01 & 1.37±0.004 \\

\hline
(3, 3, 5) &  1.27±0.013 & 0.963±0.012 & 1.086±0.012 & 0.809±0.01 & 2.062±0.01 & 1.57±0.015 & 1.841±0.006 & 1.377±0.009 \\																			
% 50 & 8.546±0.039   &   5.886±0.027 & 8.375±0.036 & 5.769±0.028 & 9.074±0.033   &   6.375±0.012 & 8.858±0.035 & 6.237±0.023 \\
\hline
\end{tabular}
\end{table*}

% \end{document}
